The Journey of CodeLab: How University Hackathons Built a Community of Engaged Students

This paper presents the journey of CodeLab: a student-organized initiative from the University of S\~ao Paulo that has grown thanks to university hackathons. It summarizes patterns, challenges, and lessons learned over 15 competitions organized by the group from 2015 to 2020. By describing these experiences, this report aims to help CodeLab to resume its events after the COVID-19 pandemic, and foster similar initiatives around the world.

==> sections/X-related_work.tex <==
\section{Related Work}\label{sec:related_work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% 1 - Hack.edu: Examining How College Hackathons Are Perceived By Student Attendees and Non-Attendees
% 2 - Hackathons as an Informal Learning Platform
% 3 - Informal STEM Learning in Game Jams, Hackathons and Game Creation Events
% 4 - Community Code Engagements: Summer of Code & Hackathons for Community Building in Scientific Software
% 5 - Digital Innovation: The Hackathon Phenomenon Gerard
% 6 - The Collegiate Hackathon Experience

There are previous works in the literature focused on the impact
of a hackathon on its participants, such as on the perception of
computing~\cite{Warner2017,Nandi2016}, on the notion of the event being an
informal learning environment~\cite{Warner2017,Nandi2016,Fowler2016}, on the
outputs produced during the event~\cite{Trainer2014}, and on the potential for
creating new connections and strengthening existing
ones~\cite{Trainer2014,Briscoe2014}.

\citet{Warner2017} studied the students' perceptions about college hackathons,
from the points of view of those who participated and those who chose not to
participate. The study found that the main motivation of the students who
attended college hackathons were both social and technical, pointing that the
format of hackathon events created an environment where learning occurred
incidentally, opportunistically, and from peers.

The importance of hackathons as an informal learning platform was also studied
by \citet{Nandi2016}. The constraints imposed by the competition format prompted
students to organize themselves in such a manner that students were able to
quickly teach and learn from their peers, improving their problem-solving,
project managing and prioritization skills. A 2-years analysis of the academic
performance of the students has shown that hackathon-participating students
have small (2--5\%) but consistently higher GPA than non-participating
students.

Ties with other participants of hackathons may depend on how students are
collocated \cite{Trainer2016} and if there is a community formed around the code
being developed, as it is the case on open-source development or hackathons for
building scientific software~\cite{Trainer2014}. The studies suggest a
trade-off  between  advancing  technical  work  and  building  social  ties,
implying that the fast-pace of hackathons and the fact that the final product is
a prototype rather than a finished product results in weaker community ties if
compared to students working on open-source development.

Studies about hackathon-like events published in major academic bases such as
ACM and IEEE focuses on the analysis of the impact of particular events on its
participants and surrounding community. Nevertheless, to the best of our
knowledge, there are no works in the literature on the long-term process of
organizing competitions and how to build a community through it.

\CodeLab members succeeded in creating a strong community around college
hackathons. In practice, this community has the same effect of open-source
communities described by \citep{Trainer2014}, allowing enduring social ties
among former participants, additionally to all benefits related to hackathons as
a learning platform.

This paper presents the outcomes of the initiative of building a multi-campus
community of students around the organization of hackathons within a university.

% Long version
% Open source communities, (non-)governmental organizations, technology companies,
% and universities organize hackathons events to promote their products, ideas and
% projects. Participants---usually students and software developers---engage on
% a fast-paced software development challenge usually designed to solve a
% real-world problem related to the organizations' goals. Hackathons are
% designed to create an environment of collaboration, innovation and fun.

% Hackathons are popular among college students and their use as an informal
% learning environment was evaluated in recent studies~\cite{Warner2017,Nandi2016,Fowler2016}.
% Students acknowledge~\cite{Warner2017} that hackathons events are fun,
% exciting opportunities where they learn from their peers.

